Disk and Envelope Structure in Class 0 Protostars: II. High Resolution Millimeter Mapping of the Serpens Sample

We present high-resolution CARMA 230 GHz continuum imaging of nine deeply embedded protostars in the Serpens Molecular Cloud, including six of the nine known Class 0 protostars in Serpens. This work is part of a program to characterize disk and envelope properties for a complete sample of Class 0 protostars in nearby low-mass star forming regions. Here we present CARMA maps and visibility amplitudes as a function of uv-distance for the Serpens sample. Observations are made in the B, C, D, and E antenna configurations, with B configuration observations utilizing the CARMA Paired Antenna Calibration System. Combining data from multiple configurations provides excellent uv-coverage (4-500 klam), allowing us to trace spatial scales from 1e2 to 1e4 AU. We find evidence for compact disk components in all of the observed Class 0 protostars, suggesting that disks form at very early times (t<0.2 Myr) in Serpens. We make a first estimate of disk masses using the flux at 50 klam, where the contribution from the envelope should be negligible, assuming an unresolved disk. The resulting disk masses range from 0.04 Msun to 1.7 Msun, with a mean of approximately 0.2 Msun. Our high resolution maps are also sensitive to binary or multiple sources with separations > 250 AU, but significant evidence of multiplicity on scales <2000 AU is seen in only one source.

==> tab1.tex <==
\ProvidesFile{tab1.tex}
\begin{deluxetable*}{llcccllcl}[width=7.8in][!hb]
%\tabletypesize{\footnotesize}
%\tabletypesize{\small}
\tablecolumns{9}
\tablewidth{0pc}
\tablecaption{Serpens Targets\label{targettab}}
\tablehead{
\colhead{ID} & \colhead{c2d name/position} & \colhead{$\mathrm{T_{bol}}$} & \colhead{$\mathrm{L_{bol}}$} & \colhead{$\mathrm{M_{env}}$} & \colhead{Class} &\colhead{Bolocam ID} & \colhead{230~GHz map?} & \colhead{Other} \\
\colhead{} & \colhead{(SSTc2dJ...)} & \colhead{(K)} & \colhead{($\mathrm{L}_{\sun}$)} & \colhead{($\mathrm{M}_{\sun}$)} & \colhead{} & \colhead{} & \colhead{} & \colhead{Names}
}
\startdata
Ser-emb 1  &  J182909.24+003132.3   &  39  &  4.1   &   3.1  &  Class 0 & Bolo 15    &  Y &  \\ 
Ser-emb 2  &  J182952.44+003611.7   &  42  &  2.5   &   1.3  &  Class 0 & Bolo 24    &  N &  \\ 
Ser-emb 3  &  J182854.84+002952.5   &  51  &  6.6   &   3.8  &  Class 0 & Bolo 8     &  N &  \\ 
Ser-emb 4  &  J183000.72+011301.4   &  54  &  3.1   &   6.6  &  Class 0 & Bolo 28    &  Y &  \\ 
Ser-emb 5  &  J182854.84+001832.6   &  56  &  0.4   &   0.5  &  Class 0 & Bolo 7     &  Y &  \\ 
Ser-emb 6  &  J182949.56+011521.9   &  56  &  28.0  &   20.0  &  Class 0 & Bolo 23    &  Y &  \object[NAME S68 FIR]{FIRS1} \\
Ser-emb 7  &  J182854.12+002929.9   &  58  &  7.9   &   4.3  &  Class 0 & Bolo 8     &  Y &  \\ %IRAS 18263+0027 
Ser-emb 8  & J182948.12+011644.9    & 58 & 5.4\tablenotemark{a} & 9.4 & Class 0 & Bolo 22 &  Y &  \object[SH 2-68 N]{S68N}  \\ 
Ser-emb 9   &  J182855.92+002944.7   &  66  &  2.5   &  6.6 &  Class 0 & Bolo 8      &  N &  \\ %IRAS 18263+0027 
Ser-emb 11  &  J182906.72+003034.3   &  77  &  4.8   &  3.6 &  Class I & Bolo 14     &  Y &  \\ %IRAS 18265+0028
Ser-emb 15  &  J182954.24+003601.3   &  100 &  0.4   &  1.3 &  Class I & Bolo 24     &  Y &  \\ %IRAS 18273+0034  \\ 
Ser-emb 17  &  J182906.36+003043.2   &  120 &  3.8   &  3.6 &  Class I & Bolo 14     &  Y &   %IRAS 18265+0028
\enddata
%\tablenotetext{a}{More than one protostar is associated with this Bolocam core}
% or source is in a crowded region; envelope mass is based on flux measured in a $30-40\arcsec$ diameter aperature.}
\tablenotetext{a}{Source is saturated at $70\micron$, so \lbol\ is likely an underestimate.}
%, but the IRAS beam is too confused to measure reliable $25\micron$ or $60\micron$ fluxes.}

\tablecomments{Position is the \textit{Spitzer} source position.  \tbol\ and \lbol\ are calculated from the broadband SED from $1.25~\micron$ to $1100~\micron$ (2MASS, IRAC, MIPS, Bolocam) and \menv\ from the total 1.1~mm flux, as described in \citet{enoch09a}.  Note that both \lbol\ and \menv\ are larger by a factor of 2.5 than those listed in \citet{enoch09a} due to the larger cloud distance assumed here.   ``Bolocam ID'' denotes the Bolocam 1.1~mm core with which the source is associated; note that more than one embedded protostar is often associated with a given Bolocam core, due to the $31\arcsec$ Bolocam resolution.  ``230 GHz map?'' indicates if the source is included in the 230~GHz study.}
\end{deluxetable*}
\endinput


==> tab2.tex <==
\ProvidesFile{tab2.tex}
\begin{deluxetable*}{llccccc}[width=7.8in][!hb]
%\tabletypesize{\footnotesize}
%\tabletypesize{\small}
\tablecolumns{7}
\tablewidth{0pc}
\tablecaption{CARMA 230~GHz source properties\label{carmatab}}
\tablehead{
\colhead{ID} & \colhead{230~GHz position} & \colhead{Peak flux} & \colhead{Total flux} & \colhead{rms} & \colhead{beam} & \colhead{deconvolved size} \\
\colhead{} & \colhead{} & \colhead{(mJy bm$^{-1}$)} & \colhead{(mJy)} & \colhead{(mJy bm$^{-1}$)} & \colhead{(arcsec)} & \colhead{(arcsec)}
}
\startdata
Ser-emb 1  &  18:29:09.09  +00:31:30.9  &  94.7  &  215  &  3.0  &  1.2$\times$1.1  &  1.5$\times$1.1  \\
%Ser-emb 4  &  18:30:00.30 +01:12:59.0  &  5.3   &  380  &  1.5  &  1.2$\times$1.1  &  12.3$\times$7.9  \\
Ser-emb 4 (N)  &  18:30:00.30  +01:12:59.4  &  6.3   &  245  &  1.5  &  1.2$\times$1.1  &  8.2$\times$6.3  \\
Ser-emb 4 (E)  &  18:30:00.70  +01:12:56.2  &  6.1   &  30.3 &  1.5  &  1.2$\times$1.1  &  2.6$\times$2.1  \\
Ser-emb 4 (S)  &  18:30:00.62  +01:12:49.5  &  5.6   &  130  &  1.5  &  1.2$\times$1.1  &  7.2$\times$4.3  \\
Ser-emb 5  &  18:28:54.91  +00:18:32.4  &  6.1   &  14.3 &  0.8  &  1.3$\times$1.2  &  1.6$\times$1.2  \\
Ser-emb 6  &  18:29:49.79  +01:15:20.4  &  423   &  1390 &  6.7  &  0.9$\times$0.9    &  1.6$\times$1.2  \\
Ser-emb 7  &  18:28:54.04  +00:29:29.7  &  9.7   &  281  &  1.9  &  1.0$\times$1.0    &  5.9$\times$4.6  \\
Ser-emb 8  &  18:29:48.07  +01:16:43.7  &  40.1  &  3970 &  4.3  &  0.7$\times$0.6    &  7.0$\times$5.9  \\
%Ser-emb 11\tablenotemark{a} &  18:29:06.63 +00:30:34.1  &  16.1  &  204  &  2.8  &  1.0$\times$1.0    &  4.4$\times$2.5  \\
Ser-emb 11 (W) &  18:29:06.61  +00:30:34.0  &  25.6  &  107  &  2.8  &  1.0$\times$1.0    &  1.9$\times$1.6  \\
Ser-emb 11 (E) &  18:29:06.75  +00:30:34.4  &  13.3  &  55.2  &  2.8  &  1.0$\times$1.0    &  1.8$\times$1.6  \\
Ser-emb 15   &  18:29:54.30  +00:36:00.8  &  41.5  &  77.5 &  1.7  &  1.0$\times$1.0    &  1.1$\times$0.8  \\
Ser-emb 17\  &  18:29:06.20  +00:30:43.1  &  42.2  &  109  &  2.8  &  1.0$\times$1.0    &  1.3$\times$1.2  
\enddata
%\tablenotetext{a}{Sources lie in the same map.}
\tablecomments{Peak fluxes, total fluxes, and source sizes are determined by a Gaussian fit in the combined 230~GHz maps.  The $1~\sigma$ rms is cacluated in the central $15\arcsec$ of each map, excluding bright sources.  An angular size of $1\arcsec$ corresponds to a physical size of 415~AU.
%[Ser-emb~4 and emb~11 have multiple sources...] 
% [restored with residual...]
}
\end{deluxetable*}
\vspace{0.2in}
\endinput


==> tab3.tex <==
\ProvidesFile{tab3.tex}
\hspace{-0.2in}
\begin{deluxetable}{lcc}[width=5.2in][!ht]
%\tabletypesize{\small}
\tablecolumns{3}
\tablewidth{0pc}
\tablecaption{Estimated disk masses\label{masstab}}
\tablehead{
\colhead{ID} &  \colhead{Flux(50~k$\lambda$)} & \colhead{Estimated \mdisk}  \\
\colhead{} & \colhead{(mJy)} & \colhead{(\msun)} 
}
\startdata
Ser-emb 1  &  120 &  0.28  \\
Ser-emb 2  &  \nodata  &  $<0.02$  \\
Ser-emb 3  &  \nodata  &  $<0.02$  \\
Ser-emb 4 (N)  &  26  &  0.05  \\
Ser-emb 5  &  17  &  0.04     \\
Ser-emb 6  &  750  &  1.7    \\
Ser-emb 7  &  66 &  0.15  \\
Ser-emb 8  &  110 &  0.25  \\
Ser-emb 9  &  \nodata  &  $<0.02$  \\
Ser-emb 11 (W) &  52  &  0.13  \\
Ser-emb 15 &  64  &  0.15  \\
Ser-emb 17 &  69  &  0.15 
\enddata
\tablecomments{The flux at 50~k$\lambda$  is the average flux for $uv$-distances $40-60$~k$\lambda$.  Disk masses are estimated from Equation~\ref{masseq}, and upper limits for Ser-emb~2, emb~3, and emb~9 are based on preliminary 110~GHz maps (Section~\ref{appendsec}).  Uncertainties in disk masses are at least 50\%, as discussed in the text.
%from absolute flux calibration uncertainties and possible envelope contributions to the flux at 50~k$\lambda$.
%, and possible errors in the visibility amplitudes due to nearby sources and extended structure. 
}
\end{deluxetable}
\endinput

